Looper: An end-to-end ML platform for product decisions

Modern software systems and products increasingly rely on machine learning models to make data-driven decisions based on interactions with users, infrastructure and other systems. For broader adoption, this practice must (i) accommodate product engineers without ML backgrounds, (ii) support finegrain product-metric evaluation and (iii) optimize for product goals. To address shortcomings of prior platforms, we introduce general principles for and the architecture of an ML platform, Looper, with simple APIs for decision-making and feedback collection. Looper covers the end-to-end ML lifecycle from collecting training data and model training to deployment and inference, and extends support to personalization, causal evaluation with heterogenous treatment effects, and Bayesian tuning for product goals. During the 2021 production deployment Looper simultaneously hosted 440-1,000 ML models that made 4-6 million real-time decisions per second. We sum up experiences of platform adopters and describe their learning curve.

==> algorithm.tex <==
% ALGORITHM STYLE -- Released 8 April 1996
%    for LaTeX-2e
% Copyright -- 1994 Peter Williams
% E-mail Peter.Williams@dsto.defence.gov.au
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithm}
\typeout{Document Style `algorithm' - floating environment}

\RequirePackage{float}
\RequirePackage{ifthen}
\newcommand{\ALG@within}{nothing}
\newboolean{ALG@within}
\setboolean{ALG@within}{false}
\newcommand{\ALG@floatstyle}{ruled}
\newcommand{\ALG@name}{Algorithm}
\newcommand{\listalgorithmname}{List of \ALG@name s}

% Declare Options
% first appearance
\DeclareOption{plain}{
  \renewcommand{\ALG@floatstyle}{plain}
}
\DeclareOption{ruled}{
  \renewcommand{\ALG@floatstyle}{ruled}
}
\DeclareOption{boxed}{
  \renewcommand{\ALG@floatstyle}{boxed}
}
% then numbering convention
\DeclareOption{part}{
  \renewcommand{\ALG@within}{part}
  \setboolean{ALG@within}{true}
}
\DeclareOption{chapter}{
  \renewcommand{\ALG@within}{chapter}
  \setboolean{ALG@within}{true}
}
\DeclareOption{section}{
  \renewcommand{\ALG@within}{section}
  \setboolean{ALG@within}{true}
}
\DeclareOption{subsection}{
  \renewcommand{\ALG@within}{subsection}
  \setboolean{ALG@within}{true}
}
\DeclareOption{subsubsection}{
  \renewcommand{\ALG@within}{subsubsection}
  \setboolean{ALG@within}{true}
}
\DeclareOption{nothing}{
  \renewcommand{\ALG@within}{nothing}
  \setboolean{ALG@within}{true}
}
\DeclareOption*{\edef\ALG@name{\CurrentOption}}

% ALGORITHM
%
\ProcessOptions
\floatstyle{\ALG@floatstyle}
\ifthenelse{\boolean{ALG@within}}{
  \ifthenelse{\equal{\ALG@within}{part}}
     {\newfloat{algorithm}{htbp}{loa}[part]}{}
  \ifthenelse{\equal{\ALG@within}{chapter}}
     {\newfloat{algorithm}{htbp}{loa}[chapter]}{}
  \ifthenelse{\equal{\ALG@within}{section}}
     {\newfloat{algorithm}{htbp}{loa}[section]}{}
  \ifthenelse{\equal{\ALG@within}{subsection}}
     {\newfloat{algorithm}{htbp}{loa}[subsection]}{}
  \ifthenelse{\equal{\ALG@within}{subsubsection}}
     {\newfloat{algorithm}{htbp}{loa}[subsubsection]}{}
  \ifthenelse{\equal{\ALG@within}{nothing}}
     {\newfloat{algorithm}{htbp}{loa}}{}
}{
  \newfloat{algorithm}{htbp}{loa}
}
\floatname{algorithm}{\ALG@name}

\newcommand{\listofalgorithms}{\listof{algorithm}{\listalgorithmname}}



==> algorithmic.tex <==
% ALGORITHMIC STYLE -- Released 8 APRIL 1996
%    for LaTeX version 2e
% Copyright -- 1994 Peter Williams
% E-mail PeterWilliams@dsto.defence.gov.au
%
% Modified by Alex Smola (08/2000)
% E-mail Alex.Smola@anu.edu.au
%
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{algorithmic}
\typeout{Document Style `algorithmic' - environment}
%
\RequirePackage{ifthen}
\RequirePackage{calc}
\newboolean{ALC@noend}
\setboolean{ALC@noend}{false}
\newcounter{ALC@line}
\newcounter{ALC@rem}
\newlength{\ALC@tlm}
%
\DeclareOption{noend}{\setboolean{ALC@noend}{true}}
%
\ProcessOptions
%
% ALGORITHMIC
\newcommand{\algorithmicrequire}{\textbf{Require:}}
\newcommand{\algorithmicensure}{\textbf{Ensure:}}
\newcommand{\algorithmiccomment}[1]{\{#1\}}
\newcommand{\algorithmicend}{\textbf{end}}
\newcommand{\algorithmicif}{\textbf{if}}
\newcommand{\algorithmicthen}{\textbf{then}}
\newcommand{\algorithmicelse}{\textbf{else}}
\newcommand{\algorithmicelsif}{\algorithmicelse\ \algorithmicif}
\newcommand{\algorithmicendif}{\algorithmicend\ \algorithmicif}
\newcommand{\algorithmicfor}{\textbf{for}}
\newcommand{\algorithmicforall}{\textbf{for all}}
\newcommand{\algorithmicdo}{\textbf{do}}
\newcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
\newcommand{\algorithmicwhile}{\textbf{while}}
\newcommand{\algorithmicendwhile}{\algorithmicend\ \algorithmicwhile}
\newcommand{\algorithmicloop}{\textbf{loop}}
\newcommand{\algorithmicendloop}{\algorithmicend\ \algorithmicloop}
\newcommand{\algorithmicrepeat}{\textbf{repeat}}
\newcommand{\algorithmicuntil}{\textbf{until}}

%changed by alex smola
\newcommand{\algorithmicinput}{\textbf{input}}
\newcommand{\algorithmicoutput}{\textbf{output}}
\newcommand{\algorithmicset}{\textbf{set}}
\newcommand{\algorithmictrue}{\textbf{true}}
\newcommand{\algorithmicfalse}{\textbf{false}}
\newcommand{\algorithmicand}{\textbf{and\ }}
\newcommand{\algorithmicor}{\textbf{or\ }}
\newcommand{\algorithmicfunction}{\textbf{function}}
\newcommand{\algorithmicendfunction}{\algorithmicend\ \algorithmicfunction}
\newcommand{\algorithmicmain}{\textbf{main}}
\newcommand{\algorithmicendmain}{\algorithmicend\ \algorithmicmain}
%end changed by alex smola

\def\ALC@item[#1]{%
\if@noparitem \@donoparitem
  \else \if@inlabel \indent \par \fi
         \ifhmode \unskip\unskip \par \fi
         \if@newlist \if@nobreak \@nbitem \else
                        \addpenalty\@beginparpenalty
                        \addvspace\@topsep \addvspace{-\parskip}\fi
           \else \addpenalty\@itempenalty \addvspace\itemsep
          \fi
    \global\@inlabeltrue
\fi
\everypar{\global\@minipagefalse\global\@newlistfalse
          \if@inlabel\global\@inlabelfalse \hskip -\parindent \box\@labels
             \penalty\z@ \fi
          \everypar{}}\global\@nobreakfalse
\if@noitemarg \@noitemargfalse \if@nmbrlist \refstepcounter{\@listctr}\fi \fi
\sbox\@tempboxa{\makelabel{#1}}%
\global\setbox\@labels
 \hbox{\unhbox\@labels \hskip \itemindent
       \hskip -\labelwidth \hskip -\ALC@tlm
       \ifdim \wd\@tempboxa >\labelwidth
                \box\@tempboxa
          \else \hbox to\labelwidth {\unhbox\@tempboxa}\fi
       \hskip \ALC@tlm}\ignorespaces}
%
\newenvironment{algorithmic}[1][0]{
\let\@item\ALC@item
  \newcommand{\ALC@lno}{%
\ifthenelse{\equal{\arabic{ALC@rem}}{0}}
{{\footnotesize \arabic{ALC@line}:}}{}%
}
\let\@listii\@listi
\let\@listiii\@listi
\let\@listiv\@listi
\let\@listv\@listi
\let\@listvi\@listi
\let\@listvii\@listi
  \newenvironment{ALC@g}{
    \begin{list}{\ALC@lno}{ \itemsep\z@ \itemindent\z@
    \listparindent\z@ \rightmargin\z@ 
    \topsep\z@ \partopsep\z@ \parskip\z@\parsep\z@
    \leftmargin 1em
    \addtolength{\ALC@tlm}{\leftmargin}
    }
  }
  {\end{list}}
  \newcommand{\ALC@it}{\addtocounter{ALC@line}{1}\addtocounter{ALC@rem}{1}\ifthenelse{\equal{\arabic{ALC@rem}}{#1}}{\setcounter{ALC@rem}{0}}{}\item}
  \newcommand{\ALC@com}[1]{\ifthenelse{\equal{##1}{default}}%
{}{\ \algorithmiccomment{##1}}}
  \newcommand{\REQUIRE}{\item[\algorithmicrequire]}
  \newcommand{\ENSURE}{\item[\algorithmicensure]}
  \newcommand{\STATE}{\ALC@it}
  \newcommand{\COMMENT}[1]{\algorithmiccomment{##1}}
%changes by alex smola
  \newcommand{\INPUT}{\item[\algorithmicinput]}
  \newcommand{\OUTPUT}{\item[\algorithmicoutput]}
  \newcommand{\SET}{\item[\algorithmicset]}
%  \newcommand{\TRUE}{\algorithmictrue}
%  \newcommand{\FALSE}{\algorithmicfalse}
  \newcommand{\AND}{\algorithmicand}
  \newcommand{\OR}{\algorithmicor}
  \newenvironment{ALC@func}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@main}{\begin{ALC@g}}{\end{ALC@g}}
%end changes by alex smola
  \newenvironment{ALC@if}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@for}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@whl}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@loop}{\begin{ALC@g}}{\end{ALC@g}}
  \newenvironment{ALC@rpt}{\begin{ALC@g}}{\end{ALC@g}}
  \renewcommand{\\}{\@centercr}
  \newcommand{\IF}[2][default]{\ALC@it\algorithmicif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\SHORTIF}[2]{\ALC@it\algorithmicif\ ##1\
    \algorithmicthen\ {##2}}
  \newcommand{\ELSE}[1][default]{\end{ALC@if}\ALC@it\algorithmicelse%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\ELSIF}[2][default]%
{\end{ALC@if}\ALC@it\algorithmicelsif\ ##2\ \algorithmicthen%
\ALC@com{##1}\begin{ALC@if}}
  \newcommand{\FOR}[2][default]{\ALC@it\algorithmicfor\ ##2\ \algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\FORALL}[2][default]{\ALC@it\algorithmicforall\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@for}}
  \newcommand{\SHORTFORALL}[2]{\ALC@it\algorithmicforall\ ##1\ %
    \algorithmicdo\ {##2}}
  \newcommand{\WHILE}[2][default]{\ALC@it\algorithmicwhile\ ##2\ %
\algorithmicdo%
\ALC@com{##1}\begin{ALC@whl}}
  \newcommand{\LOOP}[1][default]{\ALC@it\algorithmicloop%
\ALC@com{##1}\begin{ALC@loop}}
%changed by alex smola
  \newcommand{\FUNCTION}[2][default]{\ALC@it\algorithmicfunction\ ##2\ %
    \ALC@com{##1}\begin{ALC@func}}
  \newcommand{\MAIN}[2][default]{\ALC@it\algorithmicmain\ ##2\ %
    \ALC@com{##1}\begin{ALC@main}}
%end changed by alex smola
  \newcommand{\REPEAT}[1][default]{\ALC@it\algorithmicrepeat%
    \ALC@com{##1}\begin{ALC@rpt}}
    \newcommand{\UNTIL}[1]{\end{ALC@rpt}\ALC@it\algorithmicuntil\ ##1}
  \ifthenelse{\boolean{ALC@noend}}{
    \newcommand{\ENDIF}{\end{ALC@if}}
    \newcommand{\ENDFOR}{\end{ALC@for}}
    \newcommand{\ENDWHILE}{\end{ALC@whl}}
    \newcommand{\ENDLOOP}{\end{ALC@loop}}
    \newcommand{\ENDFUNCTION}{\end{ALC@func}}
    \newcommand{\ENDMAIN}{\end{ALC@main}}
  }{
    \newcommand{\ENDIF}{\end{ALC@if}\ALC@it\algorithmicendif}
    \newcommand{\ENDFOR}{\end{ALC@for}\ALC@it\algorithmicendfor}
    \newcommand{\ENDWHILE}{\end{ALC@whl}\ALC@it\algorithmicendwhile}
    \newcommand{\ENDLOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
    \newcommand{\ENDFUNCTION}{\end{ALC@func}\ALC@it\algorithmicendfunction}
    \newcommand{\ENDMAIN}{\end{ALC@main}\ALC@it\algorithmicendmain}
  } 
  \renewcommand{\@toodeep}{}
  \begin{list}{\ALC@lno}{\setcounter{ALC@line}{0}\setcounter{ALC@rem}{0}%
      \itemsep\z@ \itemindent\z@ \listparindent\z@%
      \partopsep\z@ \parskip\z@ \parsep\z@%
      \labelsep 0.5em \topsep 0.2em%
      \ifthenelse{\equal{#1}{0}}
      {\labelwidth 0.5em }
      {\labelwidth  1.2em }
      \leftmargin\labelwidth \addtolength{\leftmargin}{\labelsep}
      \ALC@tlm\labelsep
      }
    }
  {\end{list}}


